Generalizable Lightweight Proxy for Robust NAS against Diverse Perturbations

Recent neural architecture search (NAS) frameworks have been successful in finding optimal architectures for given conditions (e.g., performance or latency). However, they search for optimal architectures in terms of their performance on clean images only, while robustness against various types of perturbations or corruptions is crucial in practice. Although there exist several robust NAS frameworks that tackle this issue by integrating adversarial training into one-shot NAS, however, they are limited in that they only consider robustness against adversarial attacks and require significant computational resources to discover optimal architectures for a single task, which makes them impractical in real-world scenarios. To address these challenges, we propose a novel lightweight robust zero-cost proxy that considers the consistency across features, parameters, and gradients of both clean and perturbed images at the initialization state. Our approach facilitates an efficient and rapid search for neural architectures capable of learning generalizable features that exhibit robustness across diverse perturbations. The experimental results demonstrate that our proxy can rapidly and efficiently search for neural architectures that are consistently robust against various perturbations on multiple benchmark datasets and diverse search spaces, largely outperforming existing clean zero-shot NAS and robust NAS with reduced search cost.

==> Fig/src_plot_nasbench201.tex <==
\begin{figure}
    \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Fig/src_nasbench201/nb2cifar10_vote_ours.pdf}
         \vspace{-0.15in}
         \caption{\small{CIFAR-10}}
         \vspace{-0.1in}
         \label{fig:src_cifar10}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Fig/src_nasbench201/nb2cifar100_vote_ours.pdf}
         \vspace{-0.15in}
         \caption{\small{CIFAR-100}}
         \vspace{-0.1in}
         \label{fig:src_cifar100}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Fig/src_nasbench201/nb2im16_vote_ours.pdf}
         \vspace{-0.15in}
         \caption{\small{ImageNet16-120}}
         \vspace{-0.1in}
         \label{fig:src_imagenet}
     \end{subfigure}
    \caption{\small Spearman's rank correlation (SRC) with final test accuracy during the first 12 epochs of training on three different tasks on the NAS-Bench-201 search space. SRC for zero-cost proxies is calculated with proxy values evaluated in a random state, while EcoNAS~\citep{zhou2020econas} are calculated with validation accuracy at each epoch.}
    \label{fig:src_nasbench201}
\end{figure}


==> Table/_tbl_1_src_nasbench201_cifar10.tex <==
\begin{table}[t]
\caption{\small Comparison of Spearman's $\rho$ between the actual accuracies and the proxy values on CIFAR-10 in the NAS-Bench-201 search space. Clean stands for clean accuracy and robust accuracies are evaluated against adversarial perturbations~\cite{goodfellow2014fgsm} with various attack sizes ($\epsilon$) and common corruptions~\citep{hendrycks2019benchmarking}. Avg. stands for average Spearman's $\rho$ values with all accuracies. \textbf{Bold} and \underline{underline} stands for the best and second.}
    % \vspace{-0.15in}
    \begin{center}
    \begin{subtable}[t]{0.54\textwidth}
    
    \vspace{-0.05in}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{lcccccccca}
            \toprule
            \renewcommand{\arraystretch}{1.1}
            \renewcommand{\tabcolsep}{4pt}
            \centering
            % \multirow{3}{*}{Proxy Type} & \multicolumn{9}{c}{Spearman's rank correlation (SRC)} \\
            % \cmidrule(r){2-10}
            \multirow{2}{*}{Proxy Type} & \multirow{2}{*}{Clean} & \multicolumn{3}{c}{Adversarial Perturbation} & \multicolumn{4}{c}{Common Corruption} &\cellcolor{white} \\ 
            \cmidrule(l{2pt}r{2pt}){3-5} \cmidrule(l{2pt}r{2pt}){6-9} 
            & & $\epsilon=8$ & $\epsilon=4$ & $\epsilon=2$ & Weather & Noise & Blur & Digital & Avg.  \\
            \midrule
            \midrule
            FLOPs & 0.726 & 0.753 & 0.740 & 0.716 & 0.665 & 0.138 & 0.219 & 0.473 & 0.554 \\
            \#Params. & \underline{0.747} & 0.756 & 0.739 & 0.713 & \underline{0.674} & 0.131 & 0.215 & 0.489 & 0.558 \\
            % \cdashline{1-10}
            Plain~\cite{abdelfattah2021zero} & -0.073 & -0.059 & -0.055 & -0.029 & -0.041 & 0.048 & 0.035 & -0.032 & -0.026 \\
            Grasp~\cite{abdelfattah2021zero} & 0.440 & 0.547 & 0.563 & 0.541 & 0.459 & \underline{0.217} & 0.164 & 0.327 & 0.407 \\
            Fisher~\cite{abdelfattah2021zero} & 0.356 & 0.457 & 0.491 & 0.498 & 0.407 & \underline{0.217} & 0.221 & 0.240 & 0.361 \\
            GradNorm~\cite{abdelfattah2021zero} & 0.598 & 0.750 & \underline{0.766} & \underline{0.743} & 0.641 & \textbf{0.246} & \textbf{0.227} & 0.423 & 0.549 \\
            % Snip~\cite{abdelfattah2021zero} & 0.601 & 0.756 & \underline{0.772} & \underline{0.749} & 0.642 & \underline{0.244} & \textbf{0.228} & 0.425 & 0.385 \\
            SynFlow~\cite{abdelfattah2021zero} & 0.737 & \underline{0.778} & 
            0.750 & 0.727 & 0.673 & 0.188 & 0.165 & \underline{0.554} & \underline{0.572} \\
            % Synflow BN~\cite{abdelfattah2021zero} & 0.114 & 0.002 & 0.037 & 0.075 & 0.040 & -0.090 & 0.065 & 0.017 & 0.018 \\
            NASWOT~\cite{mellor2021neural} & 0.660 & 0.511 & 0.507 & 0.435 & 0.466 & -0.066 & -0.005 & 0.413 & 0.365 \\
            \midrule
            CRoZe & \textbf{0.823} & \textbf{0.826} & \textbf{0.801} & \textbf{0.780} & \textbf{0.743} & 0.190 & \underline{0.224} & \textbf{0.566} & \textbf{0.619} \\
            \midrule
            \bottomrule
            \end{tabular}
            }
            \vspace{-0.1in}
            \caption{Standard-Trained}
            \vspace{-0.1in}
            \label{tbl:src_nasbench201}
    \end{subtable}
    \begin{subtable}[t]{0.45\textwidth}
    
    \vspace{-0.05in}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccccc}
            \toprule
            % \centering
            % \multirow{2}{*}{Proxy Type} & \multicolumn{5}{c}{Spearman's rank correlation (SRC)} \\
            % \cmidrule(r){2-6}
            Proxy Type & Clean & FGSM & PGD & HRS(FGSM) & HRS(PGD) \\
            \midrule
            \midrule
            FLOPs & 0.670 & 0.330 & 0.418 & 0.531 & 0.515\\
            \#Params. & \underline{0.678} & 0.341 & \underline{0.429} & \underline{0.541} & \underline{0.526} \\
            % \cdashline{1-6}
            Plain~\cite{abdelfattah2021zero} & -0.042 & -0.007 & -0.012 & -0.016 & -0.016 \\
            Grasp~\cite{abdelfattah2021zero} & 0.470 & 0.324 & 0.341 & 0.392 & 0.375 \\
            Fisher~\cite{abdelfattah2021zero} & 0.482 & 0.226 & 0.276 & 0.335 & 0.334 \\
            GradNorm~\cite{abdelfattah2021zero} & 0.659 & 0.336 & 0.400 & 0.490 & 0.478\\
            % Snip~\cite{abdelfattah2021zero} & 0.665 & 0.353 & 0.679 & 0.503 & 0.491 \\
            SynFlow~\cite{abdelfattah2021zero} & 0.635 & \underline{0.355} & 0.420 & 0.519 & 0.498 \\
            % Synflow BN~\cite{abdelfattah2021zero} & 0.262 & 0.265 & 0.291 & 0.274 & 0.297 \\
            % \cdashline{2-5}
            NASWOT~\cite{mellor2021neural} & 0.600 & 0.332 & 0.381 & 0.437 & 0.438 \\
            \midrule
            CRoZe & \textbf{0.723} & \textbf{0.417} & \textbf{0.501} & \textbf{0.602} &\textbf{0.588} \\
            \midrule
            \bottomrule
            \end{tabular} }
            \vspace{-0.1in}
            \caption{Adversarially-Trained}
            \vspace{-0.1in}
            \label{tbl:src_nasbench201_fastat}
    \end{subtable}
    \vspace{-0.3in}
    \end{center}
\end{table}


==> Table/_tbl_2_src_nasbench201_otherdataset.tex <==
\begin{table}[t]
    \begin{center}
    \caption{\small Comparison of Spearman's $\rho$ between the actual accuracies and the proxy values on CIFAR-100 and ImageNet16-120 in NAS-Bench-201 search space. Avg. stands for average Spearman's $\rho$ values with all accuracies within each task. \textbf{Bold} and \underline{underline} stands for the best and second.}
    % Clean stands for clean accuracy and robust accuracies are evaluated against adversarial perturbations~\cite{goodfellow2014fgsm} and common corruptions~\citep{hendrycks2019benchmarking}. 
    \label{tbl:src_nasbench201_other}
    \resizebox{0.9\linewidth}{!}{
        \small {
        \begin{tabular}{lccccccacca}
            \toprule
            \centering
            % & \multicolumn{9}{c}{Spearman's rank correlation (SRC)} \\
            % \cmidrule{2-10}
             \multirow{2}{*}{Proxy Type} & \multicolumn{7}{c}{CIFAR-100} & \multicolumn{3}{c}{ImageNet16-120} \\
            \cmidrule(r){2-8}\cmidrule(r){9-11}
             & Clean & FGSM & Weather & Noise & Blur & Digital & Avg. & Clean & FGSM & Avg. \\ %rob = FGSM-4 
            \midrule
            \midrule
             FLOPs & 0.705 & 0.663 & 0.674  & 0.25 & 0.444 & 0.607 & 0.557 & 0.657 & 0.611 & 0.634 \\
            \#Params. & \underline{0.720} & 0.654 & 0.685 & 0.240 & 0.438 & 0.618 & 0.559 & 0.683 & 0.627 & 0.655 \\
            % \cdashline{1-11}
            Plain~\cite{abdelfattah2021zero} & -0.126 & -0.100 & -0.095 & -0.002 & -0.064 & -0.080 & -0.078 & -0.15 & -0.145 & -0.148 \\
            % Snip~\cite{abdelfattah2021zero} & 0.639 & \textbf{0.792}  & 0.655 & \underline{0.357} & \textbf{0.535} & 0.613 & \textbf{0.558} & 0.565 & 0.642 \\
            Grasp~\cite{abdelfattah2021zero} & 0.475 & 0.548 & 0.486 & \underline{0.262} & 0.374 & 0.441 & 0.431 & 0.400 & 0.437 & 0.419 \\
            Fisher~\cite{abdelfattah2021zero} & 0.378 & 0.573 & 0.419 & 0.325 & 0.435 & 0.391 & 0.420 & 0.315 & 0.388 & 0.352 \\
            GradNorm~\cite{abdelfattah2021zero} & 0.635 & \textbf{0.791} & 0.549 & \textbf{0.358} & \textbf{0.534} & 0.609 & \underline{0.579} & 0.562 & 0.643 & 0.603\\
            SynFlow~\cite{abdelfattah2021zero} & 0.769 & 0.685 & \underline{0.703} & 0.217 & 0.389 & \underline{0.642} & 0.568 & \underline{0.751} & \underline{0.695} & \underline{0.723} \\
            % Synflow BN~\cite{abdelfattah2021zero} & 0.005 & 0.054 & -0.017 & 0.033 & 0.022 & 0.032 & 0.024 & -0.345 & -0.309 \\
            % \cdashline{2-5}
            NASWOT~\cite{mellor2021neural} & 0.683 & 0.513 & 0.353 & 0.273 & 0.517 & 0.000 & 0.390 & 0.653 & 0.686 & 0.670 \\
            \midrule
            CRoZe & \textbf{0.787} & \underline{0.693} & \textbf{0.747} & 0.251 & \underline{0.450} & \textbf{0.682} & \textbf{0.602} & \textbf{0.769} & \textbf{0.696} & \textbf{0.733} \\
            \midrule
            \bottomrule
            \end{tabular} }}
            \vspace{-0.25in}
    \end{center}
\end{table}

% \begin{table}[t]
%     \begin{center}
%     \caption{\small Comparison of Spearman's rank correlation (SRC) between the actual accuracies and the proxy values on CIFAR-100 and ImageNet16-120 on NAS-Bench-201. Clean stands for clean accuracy, Rob. stands for robust accuracy evaluated against perturbed images by FGSM~\citep{jung2023neural}, and CC stands for accuracy aginst common corruption images~\citep{hendrycks2019benchmarking}.}
%     \label{tbl:src_nasbench201_other}
%     \resizebox{0.9\linewidth}{!}{
%         \small {
%         \begin{tabular}{lccccccacca}
%             \toprule
%             \centering
%             % & \multicolumn{9}{c}{Spearman's rank correlation (SRC)} \\
%             % \cmidrule{2-10}
%              \multirow{2}{*}{Proxy Type} & \multicolumn{7}{c}{CIFAR-100} & \multicolumn{2}{c}{ImageNet16-120} \\
%             \cmidrule(r){2-8}\cmidrule(r){9-10}
%              & Clean & FGSM & Weather & Noise & Blur & Digital & Avg. & Clean & FGSM & Avg. \\ %rob = FGSM-4 
%             \midrule
%             \midrule
%              FLOPs & 0.705 & 0.663 & 0.674  & 0.25 & 0.444 & 0.607 & 0.514 & 0.657 & 0.611 \\
%             \#Params. & \underline{0.720} & 0.654 & 0.685 & 0.240 & 0.438 & 0.618 & 0.514 & 0.683 & 0.627 \\
%             \cdashline{1-10}
%             Grad Norm~\cite{abdelfattah2021zero} & 0.635 & \textbf{0.791} & 0.549 & \textbf{0.358} & \textbf{0.534} & 0.609 & \textbf{0.556} & 0.562 & 0.643 \\
%             % Snip~\cite{abdelfattah2021zero} & 0.639 & \textbf{0.792}  & 0.655 & \underline{0.357} & \textbf{0.535} & 0.613 & \textbf{0.558} & 0.565 & 0.642 \\
%             Grasp~\cite{abdelfattah2021zero} & 0.475 & 0.548 & 0.486 & \underline{0.262} & 0.374 & 0.441 & 0.402 & 0.400 & 0.437 \\
%             Fisher~\cite{abdelfattah2021zero} & 0.378 & 0.573 & 0.419 & 0.325 & 0.435 & 0.391 & 0.406 & 0.315 & 0.388 \\
%             Plain~\cite{abdelfattah2021zero} & -0.126 & -0.100 & -0.095 & -0.002 & -0.064 & -0.080 & -0.071 & -0.15 & -0.145 \\
%             Synflow~\cite{abdelfattah2021zero} & 0.769 & 0.685 & \underline{0.703} & 0.217 & 0.389 & \underline{0.642} & 0.502 & \underline{0.751} & 0.695 \\
%             % Synflow BN~\cite{abdelfattah2021zero} & 0.005 & 0.054 & -0.017 & 0.033 & 0.022 & 0.032 & 0.024 & -0.345 & -0.309 \\
%             % \cdashline{2-5}
%             NASWOT~\cite{mellor2021neural} & 0.683 & 0.513 & 0.353 & 0.273 & 0.517 & 0.000 & 0.525 & 0.653 & \underline{0.686} \\
%             \midrule
%             Ours & \textbf{0.787} & \underline{0.693} & \textbf{0.747} & 0.251 & \underline{0.450} & \textbf{0.682} & \underline{0.550} & \textbf{0.769} & \textbf{0.696} \\
%             \midrule
%             \bottomrule
%             \end{tabular} }}
%             \vspace{-0.15in}
%     \end{center}
% \end{table}


% \begin{table}[t]
%     \begin{center}
%     \caption{\textbf{Efficacy of the Proposed Proxy} Comparison of Spearman's rank correlation (SRC) between the actual accuracies and the proxy values on CIFAR-100 and ImageNet16-120 on NAS-Bench-201. Clean stands for clean accuracy, Rob. stands for robust accuracy evaluated against perturbed images by FGSM~\citep{jung2023neural}, and CC stands for accuracy aginst common corruption images~\citep{hendrycks2019benchmarking}.}
%     \label{tbl:src_nasbench201_other}
%     \resizebox{\textwidth}{!}{
%     \footnotesize {
%         \begin{tabular}{c|l|ccccccccccccccc}
%             \toprule
%             \centering
%             \multirow{3}{*}{Task} & \multirow{3}{*}{Proxy Type} & \multicolumn{15}{c}{Spearman's rank correlation (SRC)} \\
%             \cmidrule(r){3-17}
%             & & \multirow{2}{*}{Clean} & \multirow{2}{*}{Rob.} & \multicolumn{3}{c}{Weather} & \multicolumn{3}{c}{Blur} & \multicolumn{3}{c}{Noise} & \multicolumn{3}{c}{Digital} & \multirow{2}{*}{CC total} \\
%             \cmidrule(r){5-7}\cmidrule(r){8-10}\cmidrule(r){11-13}\cmidrule(r){14-16}
%             & & & & Fog & Snow & Frost & Zoom & Defocus & Glass & Gaussian & Shot & Impulse & Brightness & Contrast & Jpeg \\
%             \midrule
%             \midrule
%             \multirow{11}{*}{CIFAR-100} 
%             & FLOPs & 0.705 & 0.716 & 0.706 & 0.700 & 0.588 & \textbf{0.190} & 0.377 & 0.091 & -0.018 & 0.139 & 0.294 & 0.736 & 0.451 & 0.232 & 0.514 \\
%             & \#Params. & 0.720 & 0.715 & 0.723 & \underline{0.710} & 0.588 & \underline{0.185} & \underline{0.382} & 0.077 & -0.034 & 0.126 & 0.300 & 0.757 & 0.468 & 0.241 & 0.514 \\
%             % \cdashline{2-5}
%             & Grad Norm~\cite{abdelfattah2021zero} & 0.635 & \underline{0.836} & 0.656 & 0.656 & 0.610 & 0.160 & 0.330 & \underline{0.192} & 0.122 & \textbf{0.254} & 0.363 & 0.639 & 0.404 & 0.225 & \underline{0.556} \\
%             & Snip~\cite{abdelfattah2021zero} & 0.639 & \textbf{0.837} & 0.656 & 0.659 & \underline{0.612} & 0.162 & 0.332 & 0.191 & 0.119 & \textbf{0.254} & 0.360 & 0.642 & 0.404 & 0.230 & 0.582 \\
%             & Grasp~\cite{abdelfattah2021zero} & 0.475 & 0.575 & 0.447 & 0.484 & 0.445 & 0.109 & 0.226 & 0.385 & \textbf{0.126} & \underline{0.231} & 0.294 & 0.461 & 0.263 & 0.257 & 0.402 \\
%             & Fisher~\cite{abdelfattah2021zero} & 0.378 & 0.558 & 0.407 & 0.408 & 0.407 & 0.192 & 0.248 & \textbf{0.224} & \underline{0.123} & 0.193 & 0.219 & 0.374 & 0.264 & 0.082 & 0.406 \\
%             & Plain~\cite{abdelfattah2021zero} & -0.126 & -0.114 & -0.062 & -0.048 & -0.012 & 0.047 & 0.003 & 0.055 & 0.082 & 0.061 & 0.002 & -0.064 & -0.037 & 0.005 & -0.071 \\
%             & Synflow~\cite{abdelfattah2021zero} & 0.769 & 0.771 & \underline{0.751} & 0.709 & 0.558 & 0.118 & 0.361 & 0.017 & 0.007 & 0.174 & \textbf{0.383} & \underline{0.785} & \textbf{0.513} & \textbf{0.363} & 0.502 \\
%             & Synflow BN~\cite{abdelfattah2021zero} & 0.005 & 0.017 & 0.079 & 0.058 & -0.018 & 0.071 & 0.086 & 0.037 & -0.088 & -0.116 & -0.065 & 0.087 & 0.094 & -0.131 & 0.024 \\
%             % \cdashline{2-5}
%             & NASWOT~\cite{mellor2021neural} & 0.683 & 0.607 & 0.617 & 0.494 & 0.288 & -0.078 & 0.198 & -0.135 & -0.280 & -0.139 & 0.220 & 0.619 & 0.452 & 0.169 & 0.353 \\
%             % \midrule
%             \cdashline{2-17}
%             & Ours & \textbf{0.776} & 0.774 & \textbf{0.786} & \textbf{0.782} & \textbf{0.649} & 0.188 & \textbf{0.413} & 0.075 & 0.012 & 0.185 & \underline{0.369} & \textbf{0.830} & \underline{0.511} & \underline{0.340} & 0.548 \\
%             \midrule
%             \multirow{11}{*}{ImageNet16-120} 
%             & FLOPs & 0.726 & 0.753 & 0.706 & 0.700 & 0.588 & \textbf{0.190} & 0.377 & 0.091 & -0.018 & 0.139 & 0.294 & 0.736 & 0.451 & 0.232 & 0.384 \\
%             & \#Params. & \underline{0.747} & 0.756 & 0.723 & \underline{0.710} & 0.588 & \underline{0.185} & \underline{0.382} & 0.077 & -0.034 & 0.126 & 0.300 & 0.757 & 0.468 & 0.241 & 0.387 \\
%             % \cdashline{2-5}
%             & Grad Norm~\cite{abdelfattah2021zero} & 0.598 & 0.750 & 0.656 & 0.656 & 0.610 & 0.160 & 0.330 & \underline{0.192} & 0.122 & \textbf{0.254} & 0.363 & 0.639 & 0.404 & 0.225 & 0.383 \\
%             & Snip~\cite{abdelfattah2021zero} & 0.601 & 0.756 & 0.656 & 0.659 & \underline{0.612} & 0.162 & 0.332 & 0.191 & 0.119 & \textbf{0.254} & 0.360 & 0.642 & 0.404 & 0.230 & 0.385 \\
%             & Grasp~\cite{abdelfattah2021zero} & 0.440 & 0.547 & 0.447 & 0.484 & 0.445 & 0.109 & 0.226 & 0.156 & \textbf{0.126} & \underline{0.231} & 0.294 & 0.461 & 0.263 & 0.257 & 0.289 \\
%             & Fisher~\cite{abdelfattah2021zero} & 0.356 & 0.457 & 0.407 & 0.408 & 0.407 & 0.192 & 0.248 & \textbf{0.224} & \underline{0.123} & 0.193 & 0.219 & 0.374 & 0.264 & 0.082 & 0.266 \\
%             & Plain~\cite{abdelfattah2021zero} & -0.073 & -0.059 & -0.062 & -0.048 & -0.012 & 0.047 & 0.003 & 0.055 & 0.082 & 0.061 & 0.002 & -0.064 & -0.037 & 0.005 & 0.002 \\
%             & Synflow~\cite{abdelfattah2021zero} & 0.737 & \underline{0.778} & \underline{0.751} & 0.709 & 0.558 & 0.118 & 0.361 & 0.017 & 0.007 & 0.174 & \textbf{0.383} & \underline{0.785} & \textbf{0.513} & \textbf{0.363} &\underline{0.396} \\
%             & Synflow BN~\cite{abdelfattah2021zero} & 0.114 & 0.002 & 0.079 & 0.058 & -0.018 & 0.071 & 0.086 & 0.037 & -0.088 & -0.116 & -0.065 & 0.087 & 0.094 & -0.131 & 0.018 \\
%             % \cdashline{2-5}
%             & NASWOT~\cite{mellor2021neural} & 0.660 & 0.511 & 0.617 & 0.494 & 0.288 & -0.078 & 0.198 & -0.135 & -0.280 & -0.139 & 0.220 & 0.619 & 0.452 & 0.169 & 0.206 \\
%             % \midrule
%             \cdashline{2-17}
%             & Ours & \textbf{0.816} & \textbf{0.820} & \textbf{0.786} & \textbf{0.782} & \textbf{0.649} & 0.188 & \textbf{0.413} & 0.075 & 0.012 & 0.185 & \underline{0.369} & \textbf{0.830} & \underline{0.511} & \underline{0.340} & \textbf{0.434} \\
%             \bottomrule
%             \end{tabular}\ }}
%             \vspace{-0.1in}
%     \end{center}
% \end{table}

==> Table/_tbl_3_src_nasbench201_fastat_cifar10.tex <==
\begin{table*}[t!]
    \begin{center}
    \caption{\small Comparison of Spearman's rank correlation (SRC) between the actual accuracies and the proxy values on CIFAR-10 on NAS-Bench-201. We randomly sample 500 different neural architectures in the NAS-Bench-201 dataset. Actual accuracies are obtained by evaluating the candidate architectures that are adversarially trained from scratch following~\citep{wong2020fast}. Clean stands for clean accuracy, FGSM stands for robust accuracy against FGSM, PGD-10 stands for robust accuracy against PGD-10 attack, and CC stands for accuracy against corrupted images~\citep{hendrycks2019benchmarking}.}
    \label{tbl:src_nasbench201_fastat}
    \resizebox{0.7\linewidth}{!}{
        \small {
        \begin{tabular}{l|ccccc}
            \toprule
            % \centering
            % \multirow{2}{*}{Proxy Type} & \multicolumn{5}{c}{Spearman's rank correlation (SRC)} \\
            % \cmidrule(r){2-6}
            Proxy Type & Clean & FGSM & PGD & HRS(FGSM) & HRS(PGD) \\
            \midrule
            \midrule
            FLOPs & 0.670 & 0.330 & 0.418 & 0.531 & 0.515\\
            \#Params. & \underline{0.678} & 0.341 & \underline{0.429} & \underline{0.541} & \underline{0.526} \\
            % \cdashline{2-5}
            Grad Norm~\cite{abdelfattah2021zero} & 0.659 & 0.336 & 0.678 & 0.490 & 0.478\\
            Snip~\cite{abdelfattah2021zero} & 0.665 & 0.353 & 0.679 & 0.503 & 0.491 \\
            Grasp~\cite{abdelfattah2021zero} & 0.470 & 0.324 & 0.459 & 0.392 & 0.375 \\
            Fisher~\cite{abdelfattah2021zero} & 0.482 & 0.226 & 0.463 & 0.335 & 0.334 \\
            Plain~\cite{abdelfattah2021zero} & -0.042 & -0.007 & -0.012 & -0.016 & -0.016 \\
            SynFlow~\cite{abdelfattah2021zero} & 0.635 & \underline{0.355} & 0.420 & 0.519 & 0.498 \\
            SynFlow BN~\cite{abdelfattah2021zero} & 0.262 & 0.265 & 0.291 & 0.274 & 0.297 \\
            % \cdashline{2-5}
            NASWOT~\cite{mellor2021neural} & 0.600 & 0.332 & 0.381 & 0.437 & 0.438 \\
            \midrule
            Ours & \textbf{0.723} & \textbf{0.417} & \textbf{0.501} & \textbf{0.602} &\textbf{0.588} \\
            \midrule
            \bottomrule
            \end{tabular} }
            \small
            }
            \vspace{-0.1in}
    \end{center}
\end{table*}

% \begin{table}[t]
%     \begin{center}
%     \caption{\small \textbf{Efficacy of the Proposed Proxy} Comparison of Spearman's rank correlation (SRC) between the actual accuracies and the proxy values on CIFAR-10 on NAS-Bench-201. We randomly sample 500 different neural architectures in the NAS-Bench-201 dataset. Actual accuracies are obtained by evaluating the candidate architectures that are adversarially trained from scratch following~\citep{wong2020fast}. Clean stands for clean accuracy, FGSM stands for robust accuracy against FGSM, PGD-10 stands for robust accuracy against PGD-10 attack, and CC stands for accuracy against common corruption images~\citep{hendrycks2019benchmarking}.}
%     \label{tbl:src_nasbench201_fastat}
%     \resizebox{0.7\textwidth}{!}{
%     \footnotesize {
%         \begin{tabular}{c|l|ccccc}
%             \toprule
%             \centering
%             \multirow{2}{*}{Type} & \multirow{2}{*}{Proxy Type} & \multicolumn{5}{c}{Spearman's rank correlation (SRC)} \\
%             \cmidrule(r){3-7}
%             & & Clean & FGSM & PGD-10 & CC. total  & HRS\\
%             \midrule
%             \midrule
%             \multirow{10}{*}{Baselines} 
%             & FLOPs & 0.670 & 0.330 & 0.418 & 0.404 & 0.515\\
%             & \#Params. & \underline{0.678} & 0.341 & \underline{0.429} & 0.409 & \underline{0.526} \\
%             % \cdashline{2-5}
%             & Grad Norm~\cite{abdelfattah2021zero} & 0.659 & 0.336 & 0.678 & 0.452 & 0.478\\
%             & Snip~\cite{abdelfattah2021zero} & 0.665 & 0.353 & 0.679 & \underline{0.463} & 0.491 \\
%             & Grasp~\cite{abdelfattah2021zero} & 0.470 & 0.324 & 0.459 & 0.394 & 0.375 \\
%             & Fisher~\cite{abdelfattah2021zero} & 0.482 & 0.226 & 0.463 & 0.311 & 0.334 \\
%             & Plain~\cite{abdelfattah2021zero} & -0.042 & -0.007 & -0.012 & 0.003 & -0.016 \\
%             & Synflow~\cite{abdelfattah2021zero} & 0.635 & \underline{0.355} & 0.420 & 0.421 & 0.498 \\
%             & Synflow BN~\cite{abdelfattah2021zero} & 0.262 & 0.265 & 0.291 & 0.243 & 0.297 \\
%             % \cdashline{2-5}
%             & NASWOT~\cite{mellor2021neural} & 0.600 & 0.332 & 0.381 & 0.343 & 0.438 \\
%             \midrule
%             %all sim abs
%             Ours & NAME & \textbf{0.718} & \textbf{0.411} & \textbf{0.498} & \textbf{0.475} & \textbf{0.586} \\
%             \bottomrule
%             \end{tabular}\ }}
%             \vspace{-0.1in}
%     \end{center}
% \end{table}

==> Table/_tbl_5_ablation_ours.tex <==
\begin{table*}[t!]
    \caption{Ablation study on the proposed proxy on CIFAR-10 on DARTS search space.}
    \label{tbl:ablation}
    \resizebox{0.9\textwidth}{!}{
        \begin{tabular}{ccc|cccc|ccc}
            \toprule
            \centering
            \multicolumn{3}{c}{Proxy components} & \multicolumn{4}{c}{Standard-Trained} & \multicolumn{3}{c}{Adversarially-Trained} \\
            \cmidrule(r){1-3} \cmidrule(r){4-7} \cmidrule(r){8-10}
            Parameter & Feature & Gradient & Clean & CC & FGSM & HRS & Clean & PGD-20 & HRS \\
            \midrule
            \midrule
            % allsim
            -- & $\checkmark$ & $\checkmark$ & 95.01 & 72.75 & 16.98 & \underline{28.81} & \\
            $\checkmark$ & $\checkmark$ & -- & 94.86 & \textbf{74.61} & \underline{20.57} & 22.51 & \\
            $\checkmark$ & -- & $\checkmark$ & \textbf{95.16} & 73.89 & 15.08 & 26.03 & \\
            \midrule
            $\checkmark$ & $\checkmark$ & $\checkmark$ & \underline{95.02} & \underline{74.19} & \textbf{20.68} & \textbf{33.98} & \\
            \bottomrule
    \end{tabular}}
\end{table*}


% \begin{table}[t]
%     \caption{Ablation study on the proposed proxy on CIFAR-10 on NAS-Bench-201.}
%     \label{tbl:ablation}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{ccc|ccc|cccc}
%         \toprule
%         \centering
%         &&& \multicolumn{3}{c}{Clean NAS-Bench-201~\citep{nasbench201}} & \multicolumn{4}{c}{Rob. NAS-Bench-201~\citep{jung2023neural}} \\
%         \multicolumn{3}{c}{Proxy components} & \multicolumn{3}{c}{Spearman's rank correlation (SRC)} & \multicolumn{4}{c}{Spearman's rank correlation (SRC)}\\
%         \cmidrule(r){1-3} \cmidrule(r){4-6} \cmidrule(r){7-10}
%         Parameter & Feature & Gradient & Clean & FGSM & CC & Clean & FGSM & PGD-10 & CC \\
%         \midrule
%         \midrule
%         % allsim
%         -- & $\checkmark$ & $\checkmark$ & \textbf{0.819} & \underline{0.821} & 0.432 & 0.705 & 0.406 & 0.490 & 0.471 \\
%         $\checkmark$ & $\checkmark$ & -- & 0.751 & 0.759 & 0.387 & 0.686 & 0.361 & 0.447 & 0.429 \\
%         $\checkmark$ & -- & $\checkmark$ & \textbf{0.819} & \textbf{0.823} & \textbf{0.436} & \textbf{0.730} & \textbf{0.416} & \textbf{0.502} & \textbf{0.483} \\
%         $\checkmark$ & $\checkmark$ & $\checkmark$ & \underline{0.816} & 0.820 & \underline{0.434} & \underline{0.718} & \underline{0.411} & \underline{0.498} & \underline{0.475} \\
%         \midrule
%         \midrule
%         % initw abs ablation
%         -- & $\checkmark$ & $\checkmark$ & 0.819 & 0.821 & 0.432 & 0.705 & 0.406 & 0.490 & 0.471 \\
%         $\checkmark$ & $\checkmark$ & -- & 0.823 & 0.823 & 0.430 & 0.705 & 0.402 & 0.483 & 0.469 \\
%         $\checkmark$ & -- & $\checkmark$ & \textbf{0.827} & \textbf{0.830} & \textbf{0.439} & \textbf{0.727} & \textbf{0.414} & \textbf{0.501} & \textbf{0.482} \\
%         $\checkmark$ & $\checkmark$ & $\checkmark$ & \underline{0.826} & \underline{0.829} & \underline{0.438} & \underline{0.723} & \underline{0.412} & \underline{0.500} & \underline{0.477} \\
%         \bottomrule
%     \end{tabular}}
% \end{table}


==> Table/_tbl_6_src_nasbench101_cifar10.tex <==
\begin{table}[t]
    \begin{center}
    \caption{\textbf{Efficacy of the Proposed Proxy} Comparison of Spearman's rank correlation (SRC) between the actual accuracies and the proxy values on CIFAR-10 on NAS-Bench-101.}
    \label{tbl:src_nasbench101}
    \resizebox{\textwidth}{!}{
    \footnotesize {
        \begin{tabular}{l|cccccccc|c}
            \toprule
            \centering
            & \multicolumn{8}{c}{Baselines} & \multirow{2}{*}{Ours} \\
            \cmidrule(r){2-9}
            & FLOPs & \# Params. & Grad Norm & Snip & Grasp & Fisher & Synflow & NASWOT &  \\
            \midrule
            \midrule
            NAS-Bench-101~\citep{nasbench101} & -- & 0.44 & 0.20 & 0.16 & 0.45 & 0.26 & 0.37 & 0.38 & -- \\
            \bottomrule
            \end{tabular}\ }
            }
            \vspace{-0.1in}
    \end{center}
\end{table}

==> Table/archive_e2e_clean.tex <==
\begin{table}[t]
    \begin{center}
    \caption{End-to-end performance on DARTS search space.}
    \label{tbl:e2e_darts_clean}
    \resizebox{0.7\textwidth}{!}{
        \footnotesize {
        \begin{tabular}{l|cc|cc|cc}
            \toprule
            \centering
            \multirow{2}{*}{NAS Type} & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{ImageNet16-120} \\
            \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}
             & Clean & CC & Clean & CC & Clean & CC \\
            \midrule
            \midrule 
            PC-DARTS~\citep{xu2019pc} & 95.35 & 73.62 & 76.96 & 49.95 & 50.58 & 14.36 \\
            DRNAS~\citep{chen2020drnas} & 94.64 & 72.62 & & & 49.63 & 13.42 \\
            AdvRush~\citep{mok2021advrush} & 93.53 & 72.94 & 73.51 & 46.54 & 38.72 & 10.39 \\
            \midrule
            Ours & \\
            \bottomrule
            \end{tabular}\ }}
            \vspace{-0.1in}
    \end{center}
\end{table}

==> Table/archive_e2e_darts_robustness.tex <==
\begin{table}[t]
    \begin{center}
    \caption{End-to-end performance on CIFAR-10 on DARTS search space.}
    \label{tbl:e2e_darts}
    \resizebox{\textwidth}{!}{
        \footnotesize {
        \begin{tabular}{c|l|c|cc|ccc|cc}
            \toprule
            \centering
            \multirow{2}{*}{NAS Type} & \multirow{2}{*}{Type} & \multirow{2}{*}{Model Size} & \multicolumn{2}{c}{Computational Cost (\%)} & \multicolumn{3}{c}{Adversarially Trained} & \multicolumn{2}{c}{Standard Trained} \\
            \cmidrule(r){4-5}\cmidrule(r){6-8}\cmidrule(r){9-10}
            % eps=8, alpha=2, step=20 eval
             & & &  Search Time & Memory & Clean & PGD-20 & CC & Clean & FGSM \\
            \midrule
            \midrule 
            \multirow{2}{*}{One-shot based} & RobNet-free~\cite{guo2019meets} & 5.49M & & & 82.79 & 52.74 &  \\
            & AdvRush~\cite{mok2021advrush} & 4.20M & & & 87.30 & 53.07 & & 97.58 & 55.91 \\
            % \cdashline{1-7}
            \midrule
            \multirow{2}{*}{Zero-shot based}& Synflow~\citep{abdelfattah2021zero} &  \\
            & Ours & \\
            \bottomrule
            \end{tabular}\ }}
            \vspace{-0.1in}
    \end{center}
\end{table}
